On Dominance-Free Samples of a (Colored) Stochastic Dataset

A point $p \in \mathbb{R}^d$ is said to dominate another point $q \in \mathbb{R}^d$ if the coordinate of $p$ is greater than or equal to the coordinate of $q$ in every dimension. A set of points in $\mathbb{R}^d$ is dominance-free if any two points do not dominate each other. We consider the problem of counting the dominance-free subsets of a given dataset in $\mathbb{R}^d$, or more generally, computing the probability that a random sample of a stochastic dataset in $\mathbb{R}^d$ where each point is sampled independently with its existence probability is dominance-free. In fact, we investigate a colored generalization of the problem, in which the points in the given stochastic dataset are colored and we are interested in the random samples that are inter-color dominance-free (i.e., any two points with different colors do not dominate each other). We propose the first algorithm that solves the problem for $d=2$ in near-quadratic time. On the other hand, we show that the problem is #P-hard for any $d \geq 3$, even if the points have a restricted color pattern; this implies the #P-hardness of the uncolored version (i.e., computing the dominance-free probability of a uncolored stochastic dataset) for $d \geq 3$. In addition, we show that even when the existence probabilities of the points are all equal to 0.5, the problem remains #P-hard for any $d \geq 7$; this implies the #P-hardness of counting dominance-free subsets for $d \geq 7$. In order to prove our hardness results, we establish some results about embedding the vertices a graph into low-dimensional Euclidean space such that two vertices are connected by an edge in the graph iff they form a dominance pair in the embedding. These results may be of independent interest and can possibly be applied to other problems.

==> ch-variant-csd.tex <==
\section{The free-basis colored stochastic dominance problem} \label{sec-variant}
Let $\mathcal{S} = (S,\text{cl},\pi)$ be a colored stochastic dataset in $\mathbb{R}^d$ with $S = \{a_1,\dots,a_n\}$.
%In this section, we study a variant of the CSD problem, in which the inter-color dominances are considered with respect to any orthogonal basis of $\mathbb{R}^d$.
By naturally generalizing the conventional dominance relation, one can define dominance relation with respect to a specific orthogonal basis of $\mathbb{R}^d$.
For two distinct points $p,q \in \mathbb{R}^d$ and an orthogonal basis $B = (\mathbf{b}_1,\dots,\mathbf{b}_d)$ of $\mathbb{R}^d$, we say $p$ \textit{dominates} $q$ \textit{with respect to} $B$ (denoted by $p \succ_B q$) if $\langle \mathbf{b}_i,p \rangle \geq \langle \mathbf{b}_i,q \rangle$ for every $i \in \{1,\dots,d\}$, where $\langle\cdot,\cdot\rangle$ is the inner product.
With this generalized definition, the conventional dominance relation is just dominance relation with respect to the standard basis $E = (\mathbf{e}_1,\dots,\mathbf{e}_d)$ of $\mathbb{R}^d$.
Define $\varLambda_\mathcal{S}^*$ as the probability that a realization of $\mathcal{S}$ contains inter-color dominances with respect to any orthogonal basis of $\mathbb{R}^d$.
Set $\varGamma_\mathcal{S}^* = 1 - \varLambda_\mathcal{S}^*$, which is the probability that a realization of $\mathcal{S}$ contains no inter-color dominances with respect to some orthogonal basis of $\mathbb{R}^d$.
The goal of the FBCSD problem is to compute $\varLambda_\mathcal{S}^*$ (or $\varGamma_\mathcal{S}^*$).
%We study the problem of computing $\varLambda_\mathcal{S}^*$ or $\varGamma_\mathcal{S}^*$, which we call the \textit{free-basis colored stochastic dominance} (FBCSD) problem.

\subsection{Reduction from the CSD problem} \label{sec-HDFBSD}
In this section, we show that the (standard) CSD problem in $\mathbb{R}^d$ is polynomial-time reducible to the FBCSD problem in the same dimension, which implies the latter is \#P-hard for $d \geq 3$.

Given a colored stochastic dataset $\mathcal{S} = (S,\text{cl},\pi)$ in $\mathbb{R}^d$ as an instance of the CSD problem, our reduction tries to construct another colored stochastic dataset $\mathcal{S}' = (S',\text{cl}',\pi')$ in $\mathbb{R}^d$ such that $\varLambda_{\mathcal{S}'}^*=\varLambda_\mathcal{S}$.
The intuition of our reduction is the following.
First, consider the given colored stochastic dataset $\mathcal{S}$.
Clearly, we have $\varLambda_\mathcal{S}^* \leq \varLambda_\mathcal{S}$, as every realization of $\mathcal{S}$ counted in $\varLambda_\mathcal{S}^*$ is also counted in $\varLambda_\mathcal{S}$.
The reason for why $\varLambda_\mathcal{S}^*$ may be smaller than $\varLambda_\mathcal{S}$ is that perhaps some realization contains inter-color dominances with respect to the standard basis $E$ of $\mathbb{R}^d$ but does not contain inter-color dominances with respect to some other basis.
To handle this, our basic idea is to add a set $\varPsi$ of (colored) auxiliary points with existence probabilities 1 to $S$, that is, we want $S' = S \cup \varPsi$ with $\pi'(b) = 1$ for all $b \in \varPsi$ (and $\pi'(a) = \pi(a)$, $\text{cl}'(a) = \text{cl}(a)$ for all $a \in S$).
The goal of adding these auxiliary points is to guarantee that a subset $A \subseteq S$ contains inter-color dominances with respect to the standard basis $E$ iff $A \cup \varPsi \subseteq S'$ contains inter-color dominances with respect to any orthogonal basis.
Note that as long as $\varPsi$ has this property, it obviously holds that $\varLambda_{\mathcal{S}'}^*=\varLambda_\mathcal{S}$.
Therefore, the critical part of our reduction is to construct such a set $\varPsi$ with the desired property.
%It is not difficult to make $\varPsi$ satisfy the ``if'' condition, i.e., $R \subseteq S$ contains inter-color dominances with respect to $E$ if $R \cup \varPsi$ contains inter-color dominances with respect to every orthogonal basis.
%We only need to guarantee that the auxiliary points in $\varPsi$ do not dominate each other and have no dominance relation with any points in $S$, with respect to $E$.
%The tricky part is to make $\varPsi$ satisfy the ``only if'' condition.
We achieve this through several steps.

First of all, we need to make the point set $S$ ``regular''.
%The first step is to ``regularize'' the point set $S$.
Formally, we say a (finite) point set $X \subset \mathbb{R}^d$ is \textit{regular} if $X \subset \{1,2,\dots,|X|\}^d$ and any two distinct points $x,x' \in X$ have distinct coordinates in all dimensions.
It is easy to see that one can always ``regularize'' a point set without changing the dominance relation (with respect to $E$) among the points.
\begin{lemma} \label{lem-regular}
    Given a set $S = \{a_1,\dots,a_n\} \subset \mathbb{R}^d$ of distinct points, one can construct in $O(n \log n)$ time a regular set $S_{new} = \{\hat{a}_1,\dots,\hat{a}_n\} \subset \mathbb{R}^d$ such that $\hat{a}_i \succ_E \hat{a}_j$ iff $a_i \succ_E a_j$.
\end{lemma}
Now we may assume $S$ is regular.
To construct $\varPsi$, we need to introduce some notions.
\begin{definition}
    Let $B = (\mathbf{b}_1,\dots,\mathbf{b}_d)$ be an orthogonal basis of $\mathbb{R}^d$.
    We define the \textit{cone} $C_B$ of $B$ as
    \begin{equation*}
        C_B = \left\{\sum_{i=1}^{d} \beta_i \mathbf{b}_i: \beta_1,\dots,\beta_d \geq 0\right\} \cup \left\{\sum_{i=1}^{d} \beta_i \mathbf{b}_i: \beta_1,\dots,\beta_d \leq 0\right\} \subset \mathbb{R}^d.
    \end{equation*}
    Also, we define the \textit{projective cone} $\mathit{PC}_B \subset \mathbb{P}^{d-1}$ as the image of $C_B \backslash \{\mathbf{0}\}$ in $\mathbb{P}^{d-1}$ under the obvious quotient map $\mathbb{R}^d \backslash \{\mathbf{0}\} \rightarrow \mathbb{P}^{d-1}$.
\end{definition}
For a point $x \in \mathbb{R}^d$ with $x \neq \mathbf{0}$, we denote by $\overline{x}$ its image in $\mathbb{P}^{d-1}$ under the quotient map $\mathbb{R}^d \backslash \{\mathbf{0}\} \rightarrow \mathbb{P}^{d-1}$.
The notion of (projective) cone defined above gives us another way to view dominance relations with respect to an orthogonal basis.
Consider two distinct points $p,q \in \mathbb{R}^d$, and an orthogonal basis $B$ of $\mathbb{R}^d$.
It is easy to see that $p,q$ form a dominance with respect to $B$ (i.e., $p \succ_B q$ or $q \succ_B p$) iff $p-q \in C_B$, or equivalently, $\overline{p-q} \in \mathit{PC}_B$.
Another notion we need is a metric on any projective space $\mathbb{P}^k$.
\begin{definition}
    For two points $l,l' \in \mathbb{P}^k$, we define $\textnormal{ang}(l,l') \in [0,\frac{\pi}{2}]$ to be the angle between $l$ and $l'$ as lines in $\mathbb{R}^{k+1}$ through the origin \textnormal{(}there are two supplementary angles, take the smaller one which is in $[0,\frac{\pi}{2}]$\textnormal{)}.
    It is easy to see that $\textnormal{ang}(\cdot,\cdot)$ defines a metric on $\mathbb{P}^k$.
\end{definition}
The following lemmas establish some geometric properties of the projective cone and the $\text{ang}$-metric, which will be helpful for constructing $\varPsi$.
\begin{lemma} \label{lem-con1}
    Let $B$ be an orthogonal basis of $\mathbb{R}^d$, and $l$ be a point in $\mathbb{P}^{d-1}$.
    If $l \notin \mathit{PC}_B$, then there exists $x \in \mathit{PC}_B$ perpendicular to $l$, i.e., $\textnormal{ang}(l,x)=\frac{\pi}{2}$.
\end{lemma}
\begin{lemma} \label{lem-con2}
    %There exists a constant $c$ satisfying the following property:
    For any orthogonal basis $B$ of $\mathbb{R}^d$, any point $x \in \mathit{PC}_B$, and any real number $\varepsilon \in (0,\frac{\pi}{2}]$, there exists $y \in \mathit{PC}_B$ with $\textnormal{ang}(x,y)<\varepsilon$ such that the $\frac{\varepsilon}{3\sqrt{d}}$-ball at $y$, i.e., the set $\{z \in \mathbb{P}^{d-1}: \textnormal{ang}(z,y) \leq \frac{\varepsilon}{3\sqrt{d}}\}$, is contained in $\mathit{PC}_B$.
    %The constant $c$ only depends on the dimension $d$.
    %Let $l$ be a point in $\mathbb{P}^{d-1}$.
    %If $B$ is an orthogonal basis of $\mathbb{R}^d$ with $l \in \mathit{PC}_B$, then for any real number $\varepsilon \in (0,\frac{\pi}{2}]$, there exist $l' \in \mathit{PC}_B$ and $\xi = \Omega(\varepsilon)$ such that the $\xi$-ball at $l'$ is contained in $\mathit{PC}_B$ and $\textnormal{ang}(l,l')<\varepsilon$.
\end{lemma}
\begin{lemma} \label{lem-net}
    Let $l$ be a point in $\mathbb{P}^{d-1}$ and $\varepsilon \geq \xi > 0$ be two real numbers.
    %Set $L = \{l' \in \mathbb{P}^{d-1}: \textnormal{ang}(l,l')>\frac{\pi}{2}-\varepsilon\}$.
    Then one can compute $m = O(\varepsilon/\xi^{d-1})$ points $l_1,\dots,l_m \in \mathbb{P}^{d-1}$ in $O(m)$ time such that \textnormal{(1)} $\textnormal{ang}(l,l_i)>\frac{\pi}{2}-\varepsilon$ for all $i \in \{1,\dots,m\}$ and \textnormal{(2)} for any $y \in \mathbb{P}^{d-1}$ with $\textnormal{ang}(l,y)>\frac{\pi}{2}-\varepsilon$, there exists some $l_i$ satisfying $\textnormal{ang}(l_i,y)<\xi$.
\end{lemma}

With the above lemmas in hand, we now describe the construction of $\varPsi$.
%According to Lemma~\ref{lem-con2}, we may choose a small enough constant $c$ such that for any $\varepsilon \in (0,\frac{\pi}{2}]$ there exists $\delta \geq c\varepsilon$ satisfying the condition in the lemma.
We look at all pairs $(a,a')$ of points in $S$ such that $\text{cl}(a) \neq \text{cl}(a')$ and $a \succ_E a'$.
For each such pair $(a,a')$, we do the following.
Set $l = \overline{a-a'} \in \mathbb{P}^{d-1}$, $\varepsilon = \arcsin(\frac{1}{\sqrt{d}n})$, and $\xi = \frac{\varepsilon}{3\sqrt{d}}$.
By applying Lemma~\ref{lem-net} with $l,\varepsilon,\xi$, we compute $m = O(\varepsilon/\xi^{d-1}) = O(n^{d-2})$ points $l_1,\dots,l_m \in \mathbb{P}^{d-1}$ satisfying the conditions (1) and (2) in the lemma.
In addition, we observe the following. \\
$\bullet$ $l_i \notin \mathit{PC}_E$ for all $i \in \{1,\dots,m\}$. \\
$\bullet$ For any orthogonal basis $B$ of $\mathbb{R}^d$, if $l \notin \mathit{PC}_B$, then there exists some $l_i \in \mathit{PC}_B$. \\
To see the first observation, recall that $S$ is already regular.
Since $a \succ_E a'$ and $S$ is regular, $l$ can be represented by homogeneous coordinates $[\alpha_1:\dots:\alpha_d]$ with $\alpha_1,\dots,\alpha_d \in \{1,\dots,n-1\}$.
Based on this, one can easily verify that $\text{ang}(l,l')<\arccos(\frac{1}{\sqrt{d}n})$ for any $l' \in \mathit{PC}_E$.
But we have $\textnormal{ang}(l,l_i)>\frac{\pi}{2}-\varepsilon=\arccos(\frac{1}{\sqrt{d}n})$ by Lemma~\ref{lem-net}.
Thus, $l_i \notin \mathit{PC}_E$.
To see the second observation, let $B$ be an orthogonal basis of $\mathbb{R}^d$ with $l \notin \mathit{PC}_B$.
By Lemma~\ref{lem-con1}, there exists $x \in \mathit{PC}_B$ with $\textnormal{ang}(l,x)=\frac{\pi}{2}$.
Then by Lemma~\ref{lem-con2}, there exists $y \in \mathit{PC}_B$ such that $\textnormal{ang}(x,y)<\varepsilon$ and the $\frac{\varepsilon}{3\sqrt{d}}$-ball at $y$ is contained in $\mathit{PC}_B$.
Since $\textnormal{ang}(l,x)=\frac{\pi}{2}$ and $\textnormal{ang}(x,y)<\varepsilon$, we have $\textnormal{ang}(l,y)>\frac{\pi}{2}-\varepsilon$.
Therefore, according to the condition (2) in Lemma~\ref{lem-net}, there must exist some $l_i$ such that $\textnormal{ang}(l_i,y)<\xi$.
Recall that $\xi = \frac{\varepsilon}{3\sqrt{d}}$, so $l_i$ is in the $\frac{\varepsilon}{3\sqrt{d}}$-ball at $y$ and hence in $\mathit{PC}_B$.
These two observations will be used later to verify that $\varPsi$ satisfies the desired property.
Now we continue to discuss the construction of $\varPsi$.
We have computed $m$ points $l_1,\dots,l_m \in \mathbb{P}^{d-1}$ for a specific pair $(a,a')$.
We do the same thing for all pairs $(a,a')$ of points in $S$ with $\text{cl}(a) \neq \text{cl}(a')$ and $a \succ_E a'$.
After this, we obtain $M = O(n^2m) = O(n^d)$ points in $\mathbb{P}^{d-1}$ (with an abuse of notation, we denote them by $l_1,\dots,l_M$).
The set $\varPsi$ we construct consists of $2M$ points $b_1,\dots,b_M,b_1',\dots,b_M' \in \mathbb{R}^d$ where $b_i,b_i'$ correspond to $l_i$ for $i \in \{1,\dots,M\}$.
We set the coordinates of each $b_i$ in $\mathbb{R}^d$ to be $(-i,\dots,-i,n+i)$.
Then we choose location for each $b_i'$ in $\mathbb{R}^d$ such that $\lVert b_i'-b_i\rVert_2 < 0.1$ and $\overline{b_i'-b_i} = l_i$ (there are infinitely many choices, we arbitrarily pick one of them).
Finally, we need to define the coloring of the points in $\varPsi$, i.e., $\text{cl}'(b)$ for all $b \in \varPsi$.
We arbitrarily color the points in $\varPsi$ under the only restriction that $b_i$ and $b_i'$ must have different colors, i.e., $\text{cl}'(b_i) \neq \text{cl}'(b_i')$, for all $i \in \{1,\dots,M\}$.
It suffices to verify the property that $A \subseteq S$ contains inter-color dominances with respect to $E$ iff $A \cup \varPsi \subseteq S'$ contains inter-color dominances with respect to any orthogonal basis.
To see the ``if'' part, let $A \subseteq S$ be a subset such that $A \cup \varPsi \subseteq S'$ contains inter-color dominances with respect to any orthogonal basis.
Since $S \subset [1,n]^d$ (as $S$ is regular) and $l_i \notin \mathit{PC}_E$ for all $i \in \{1,\dots,M\}$ (as observed above), the points in $\varPsi$ do not dominate each other and do not form dominance with any points in $S$, with respect to $E$.
But by assumption, $A \cup \varPsi$ contains inter-color dominances with respect to $E$.
So the inter-color dominances must be formed by the points in $A$, i.e., $A$ contains inter-color dominances with respect to $E$.
To see the ``only if'' part, let $A \subseteq S$ be a subset containing inter-color dominances with respect to $E$.
Suppose $a,a' \in A$ are two points such that $\text{cl}(a) \neq \text{cl}(a')$ and $a \succ_E a'$.
Consider an orthogonal basis $B$ of $\mathbb{R}^d$, and we must show that $A \cup \varPsi$ contains inter-color dominances with respect to $B$.
If $a \succ_B a'$ or $a' \succ_B a$, then we are done.
Otherwise, recall that we have $m$ points in $\{l_1,\dots,l_M\}$ which are chosen for the pair $(a,a')$ (assume they are $l_1,\dots,l_m$ without loss of generality).
By our observation above, one of these $m$ points must be in $\mathit{PC}_B$, say $l_1 \in \mathit{PC}_B$.
Then the two points $b_1,b_1' \in \varPsi$ form an inter-color dominance with respect to $B$.

By the above construction, we obtain a colored stochastic dataset $\mathcal{S}' = (S \cup \varPsi,\text{cl}',\pi')$ in $\mathbb{R}^d$ satisfying $\varLambda_{\mathcal{S}'}^*=\varLambda_\mathcal{S}$.
Clearly, this reduction can be done in polynomial time.
Thus, the FBCSD problem is \#P-hard for $d \geq 3$.
In fact, with some efforts, one can make this result stronger by considering the FBCSD problem with respect to a balanced color pattern.
\begin{theorem} \label{thm-FBCSD-hard}
    Let $\mathcal{P}' = (\varDelta_1',\varDelta_2',\dots)$ be a balanced color pattern.
    Then for any fixed $d$, there exists a balanced color pattern $\mathcal{P} = (\varDelta_1,\varDelta_2,\dots)$ such that the CSD problem in $\mathbb{R}^d$ with respect to $\mathcal{P}$ is polynomial-time reducible to the FBCSD problem in $\mathbb{R}^d$ with respect to $\mathcal{P}'$.
    In particular, the FBCSD problem in $\mathbb{R}^d$ with respect to $\mathcal{P}'$ is \#P-hard for $d \geq 3$.
\end{theorem}

\subsection{Reduction to the CSD problem for \texorpdfstring{$d=2$}{d=2}}
In this section, we study the FBCSD problem for $d=2$ and show that an instance of the FBCSD problem in $\mathbb{R}^2$ can be reduced to $O(n^2)$ instances of the CSD problem in $\mathbb{R}^2$.
By combining this reduction with our algorithm given in Section~\ref{sec-2DSD}, we directly obtain an $O(n^4 \log^2 n)$-time algorithm for the FBCSD problem in $\mathbb{R}^2$.
For simplicity of exposition, we assume that $S$ is in general position in $\mathbb{R}^2$, i.e., no three points are collinear.


We try to compute $\varGamma_\mathcal{S}^*$.
When computing $\varGamma_\mathcal{S}^*$, we need to consider the realizations of $\mathcal{S}$ which contain no inter-color dominances with respect to some orthogonal basis of $\mathbb{R}^2$ (these realizations are said to be \textit{good}).
%Let $R \subseteq S$ be a subset.
We first establish a criterion for testing whether a realization is good.
Recall that for a nonzero point $x \in \mathbb{R}^d$, the notation $\overline{x}$ denotes the image of $x$ in $\mathbb{P}^{d-1}$ under the quotient map $\mathbb{R}^d \backslash \{\mathbf{0}\} \rightarrow \mathbb{P}^{d-1}$.
For a subset $A \subseteq S$, we define $L_A = \{\overline{a_i-a_j}:a_i,a_j \in A \text{ and } \text{cl}(a_i) \neq \text{cl}(a_j)\} \subset \mathbb{P}^1$.
For two points $l,l' \in \mathbb{P}^1$, we denote by $\theta(l,l')$ the angle between $l$ and $l'$ whose counterclockwise boundary is $l$ and clockwise boundary is $l'$ (when talking about angle we regard $l$ and $l'$ as lines in $\mathbb{R}^2$ through the origin).
\begin{wrapfigure}{r}{4cm}
    \centering
    \includegraphics[height=3.5cm]{fbcsd.pdf}
    \caption{An example of witness pair.
        $l = \overline{a_1 - a_8} = \overline{a_2 - a_5}$.
        $\text{wit}(R) = (a_1, a_8)$.
    }
    \label{figure:witness}
    \vspace{-25pt}
\end{wrapfigure}
Then we have the following observation.
\begin{lemma} \label{lem-criterion}
    A realization $R$ of $\mathcal{S}$ is good iff $L_R = \emptyset$ or there exists a unique $l \in L_R$ such that $\theta(l,l') > \frac{\pi}{2}$ for any $l' \in L_R$ not equal to $l$.
\end{lemma}
Note that $L_R = \emptyset$ iff $R$ is monochromatic.
Based on the above lemma, we now define a notion called \textit{witness pair} as follows.
Let $R$ be a good but not monochromatic realization of $\mathcal{S}$.
Then by Lemma~\ref{lem-criterion}, there exists a unique $l \in L_R$ such that $\theta(l,l') > \frac{\pi}{2}$ for any $l' \in L_R$ not equal to $l$.
According to the definition of $L_R$, we must have $l = \overline{a_i-a_j}$ for some $a_i,a_j \in R$ with $\text{cl}(a_i) \neq \text{cl}(a_j)$.
Note that the choice of $a_i,a_j$ is not necessarily unique (though $l$ is unique).
Let $Y$ be the set of all pairs $(a_i,a_j)$ with $a_i,a_j \in R$ satisfying $\text{cl}(a_i) \neq \text{cl}(a_j)$ and $l = \overline{a_i-a_j}$.
We claim that there exists a unique pair $(a_{i^*},a_{j^*}) \in Y$ such that for any $(a_i,a_j) \in Y$ we have $j^* \geq j$.
The existence is obvious, so it suffices to show the uniqueness.
Indeed, if $(a_i,a_j)$ and $(a_{i'},a_j)$ are two pairs in $Y$, then the points $a_i,a_{i'},a_j$ must be collinear in $\mathbb{R}^2$.
However, because of the general position assumption for $S$ (and hence for $R$), we must have $i = i'$.
It follows that for any $j \in \{1,\dots,n\}$ there is at most one pair $(a_i,a_j) \in Y$, which further implies the uniqueness of $(a_{i^*},a_{j^*})$.
We define the pair $(a_{i^*},a_{j^*})$ as the \textit{witness pair} of $R$, denoted by $\text{wit}(R)$.
See Figure~\ref{figure:witness} for an example.
Now it is clear that
\begin{equation*}
    \varGamma_S^* = \mathit{Pr}_\text{mono} + \sum_{i=1}^{n} \sum_{j=1}^{n} \mathit{Pr}_{i,j},
\end{equation*}
where $\mathit{Pr}_\text{mono}$ is the probability that a realization $R$ of $\mathcal{S}$ is monochromatic, and $\mathit{Pr}_{i,j}$ is the probability that $R$ is good (but not monochromatic) with $\text{wit}(R) = (a_i,a_j)$.

It is easy to compute $\mathit{Pr}_\text{mono}$ in linear time.
The problem remaining is how to compute $\mathit{Pr}_{i,j}$ for all $i,j \in \{1,\dots,n\}$.
Fix a pair $(i^*,j^*)$.
Obviously, if $\text{cl}(a_{i^*}) = \text{cl}(a_{j^*})$, we immediately have $\mathit{Pr}_{i^*,j^*}=0$.
So suppose $\text{cl}(a_{i^*}) \neq \text{cl}(a_{j^*})$.
We try to reduce the the task of computing $\mathit{Pr}_{i^*,j^*}$ to an instance of the CSD problem in $\mathbb{R}^2$.
Let $\mathbf{b}_1 = (a_{i^*}-a_{j^*})/ \lVert a_{i^*}-a_{j^*} \rVert_2$ be a unit vector of $\mathbb{R}^2$, and $\mathbf{b}_2$ be another unit vector obtained by rotating $\mathbf{b}_1$ clockwise with angle $\frac{\pi}{2}$.
Clearly, $B = (\mathbf{b}_1,\mathbf{b}_2)$ is an orthogonal basis of $\mathbb{R}^2$.
We define $n$ points $a_1',\dots,a_n' \in \mathbb{R}^2$ as follows.
Let $\delta$ be a small enough real number such that for any $i,j \in \{1,\dots,n\}$ we have $|\langle \mathbf{b}_2,a_i \rangle - \langle \mathbf{b}_2,a_j \rangle| > \delta$ unless $\langle \mathbf{b}_2,a_i \rangle = \langle \mathbf{b}_2,a_j \rangle$.
Consider a specific index $p \in \{1,\dots,n\}$.
If $p \leq j^*$ and there exists $q \leq j^*$ satisfying $\text{cl}(a_p) \neq \text{cl}(a_q)$, $a_p \succ_B a_q$, $\langle \mathbf{b}_2,a_p \rangle = \langle \mathbf{b}_2,a_q \rangle$, then we set the coordinates of $a_p'$ in $\mathbb{R}^2$ to be $(\langle \mathbf{b}_2,a_p \rangle - \delta, \langle \mathbf{b}_1,a_p \rangle)$.
Otherwise, we set the coordinates of $a_p'$ to be $(\langle \mathbf{b}_2,a_p \rangle, \langle \mathbf{b}_1,a_p \rangle)$.
Based on this, we can construct a colored stochastic dataset $\mathcal{S}' = (S',\text{cl}',\pi')$ in $\mathbb{R}^2$ by defining $S' = \{a_1',\dots,a_n'\}$, $\text{cl}'(a_i') = \text{cl}(a_i)$ for all $i \in \{1,\dots,n\}$, and
$\pi'(a_{i^*}') = \pi'(a_{j^*}') = 1$, $\pi'(a_i') = \pi(a_i)$ for all
$i \in \{1, \dots, n\} \backslash \{i^*, j^*\}$.
%\begin{equation*}
%    \pi'(a_i') = \left\{
%    \begin{array}{ll}
%        1 & \text{if } i = i^* \text{ or } i = j^*, \\
%        \pi(a_i) & \text{otherwise}.
%    \end{array}
%    \right.
%\end{equation*}
We observe the following equation, which allows us to compute $\mathit{Pr}_{i^*,j^*}$ by solving the instance $\langle \mathcal{S}' \rangle$ of the CSD problem in $\mathbb{R}^2$.
\begin{lemma} \label{lem-equation}
    $\mathit{Pr}_{i^*,j^*} = \pi(a_{i^*}) \cdot \pi(a_{j^*}) \cdot \varGamma_{\mathcal{S}'}$.
\end{lemma}
%It follows that we can compute $\mathit{Pr}_{i^*,j^*}$ by solving the instance $\langle \mathcal{S}' \rangle$ of the CSD problem in $\mathbb{R}^2$.
In this way, an instance of the FBCSD problem in $\mathbb{R}^2$ is reduced to $O(n^2)$ instances of the CSD problem in $\mathbb{R}^2$.
By plugging in our $O(n^2 \log^2 n)$ algorithm for solving the CSD problem in $\mathbb{R}^2$, we have the following result.
\begin{theorem}
    The FBCSD problem in $\mathbb{R}^2$ can be solved in $O(n^4 \log^2 n)$ time.
\end{theorem}

==> figure_page.tex <==
\section*{Figure Page}

\begin{figure}[h]
    \centering
    \includegraphics[height=3cm]{csd-Z.pdf}
    \caption{Illustrating $A$ and $Z(A)$.}
    \label{figure:A_and_Z(A)}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[height=3cm]{st-dom-fig-2a}
    \caption{Inserting new vertices to each edge of $G$.}
    \label{fig-2a}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[height=2.5cm]{st-dom-fig-2b}
    \caption{An orthogonal grid drawing.}
    \label{fig-2b}
\end{figure}

\begin{figure}[H]
    \centering
    \subfloat[]{
        \includegraphics[height=2.5cm]{st-dom-fig-2c-1.pdf}
        \label{figure:2c-1}
    }
    \hspace{1cm}
    \subfloat[]{
        \includegraphics[height=2.5cm]{st-dom-fig-2c-2.pdf}
        \label{figure:2c-2}
    }
    \hspace{1cm}
    \subfloat[]{
        \includegraphics[height=2.5cm]{st-dom-fig-2c-3.pdf}
        \label{figure:2c-3}
    }
    \caption{The construction of $P_e$.}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[height=3.5cm]{fbcsd.pdf}
    \caption{An example of witness pair.
        $l = \overline{a_1 - a_8} = \overline{a_2 - a_5}$.
        $\text{wit}(R) = (a_1, a_8)$.
    }
    \label{figure:witness}
\end{figure}
